Safety in the Emerging Holodeck Applications

Technological advances in holography, robotics, and 3D printing are starting to realize the vision of a holodeck. These immersive 3D displays must address user safety from the start to be viable. A holodeck's safety challenges are novel because its applications will involve explicit physical interactions between humans and synthesized 3D objects and experiences in real-time. This pioneering paper first proposes research directions for modeling safety in future holodeck applications from traditional physical human-robot interaction modeling. Subsequently, we propose a test-bed to enable safety validation of physical human-robot interaction based on existing augmented reality and virtual simulation technology.

==> newdisplay.tex <==


\begin{algorithm}
\caption{MinDist
%A point assignment and deployment heuristic to minimize travel distance.  The second for loop may be processed by each dispatcher in parallel with other dispatchers.
}\label{alg:mindist}
\begin{small}
  \For{$i\gets1$ \KwTo $\alpha$ \KwBy $1$\Comment*[r]{Iterate $\alpha$ points}}{
    $min \gets MaxInteger$\;
    \For{$j \gets1$ \KwTo $\psi$ \KwBy $1$\Comment*[r]{Iterate $\psi$ dispatchers}}{
        $\Delta \gets$ Distance ($Point_i$, $Dispatch_j$)\;
        \If{$\Delta < min$}
        {
        $min \gets \Delta$\;
        $tgt \gets j$\;
        }
    }
    $Dispatch_{tgt} \gets Point_i$\;
    }
    \For{$j \gets1$ \KwTo $\psi$ \KwBy $1$\Comment*[r]{Deploy FLSs}}{
    $Dispatch_j$ sorts its points in descending distance order\;
    $Dispatch_j$ deploys points starting with the farthest away one\;
    }
    \end{small}
\end{algorithm}

MinDist has several limitations.  First, it may result in a slow rendering of an illumination by utilizing a subset of dispatchers more often than others.  This happens when most of the points in a cloud are clustered in close proximity of a few dispatchers.
While these dispatchers deploy most of the FLSs sequentially, other dispatchers sit idle.
See discussions of Table~\ref{tbl:staticCMP} in Section~\ref{sec:staticeval}.

Second, MinDist assumes a dispatcher may access all hangars and their FLSs.  This assumption is violated when hangars are physically partitioned across dispatchers.  MinDist may not render an illumination that consists of a cluster of points in close proximity of a dispatcher with insufficient number of FLSs.

We now present Alg~\ref{alg:balance}, QuotaBlanced, that considers the distance travelled by FLSs, FLS speed, the number of dispatchers, the number of FLSs accessible to a dispatcher, and the rate at which a dispatcher may deploy FLSs.
It assigns a quota to each dispatcher that is reduced as a function of the travel time by its deployed FLSs.  The idea is to have a dispatcher that is very far from the points of a cloud to deploy some FLSs but not as many FLSs as those dispatchers that are in close proximity to the points of the cloud. 

\begin{algorithm}
\caption{QuotaBalanced
%A point assignment to minimize time required to render an illumination.
}\label{alg:balance}
\begin{small}
  $f \gets FLS~deployment~rate, \frac{FLSs}{second}$\;
  $S \gets FLS~Speed$\;
  $\varpi[1..\psi] \gets \frac{\alpha}{\psi \times f}$\Comment*[r]{Quota for each dispatcher}
  $\{Active\} \gets Dispatchers~with~FLSs~and~quota~>~0$\;
  \For{$i\gets1$ \KwTo $\alpha$ \KwBy $1$}{
  %\Comment{Lines~1-13~of~Alg~\ref{alg:mindist} compute $Dispatch_{tgt}$.}
    $Dispatch_{tgt} \gets$ The active dispatcher closest to $Point_i$\;





    }

    \For{$j \gets1$ \KwTo $\psi$ \KwBy $1$}{
    $Dispatch_j$ sorts its points in descending distance order\;
    $Dispatch_j$ deploys points starting with the farthest away one\;
    }
\end{small}
\end{algorithm}

Distance is an approximation of travel time.  The time for an FLS to fly from a dispatcher to its display cell is a function of the FLS speed.
A dispatcher may be far from the point cloud.  However, if FLSs are extremely fast then their travel time may become insignificant to the time to deploy FLSs.
This motivates an algorithm that requires each dispatcher to deploy its fair share\footnote{This changes the problem definition.  We are no longer minimizing total distance travelled.} of FLSs while considering travel time of FLSs.  QuotaBalanced is one such algorithm. 

QuotaBalanced assumes each dispatcher may deploy $f$ FLSs per time unit (Line 1 of Alg~\ref{alg:balance}) and dispatcher $i$ has access to a fixed number of FLSs.  The granularity of its quota is time units required for a dispatcher to deploy its fair share of FLSs for the point cloud, $\frac{\alpha}{\psi \times f}$.  This algorithm converts distance to time using the speed of an FLS, see Line 12.

%%QuotaBalanced continues to use minimum distance to assign points to a dispatcher.  

In each iteration, QuotaBalanced reduces the quota of a dispatcher by the FLS travel time to its assigned point.  Once the quota of a disptacher is exhausted, it is removed from the list of active dispatchers.  This causes QuotaBalanced to assign points to other dispatchers that are not necessarily as close.  However, the quota of these dispatchers are reduced by a larger value because they are farther away, i.e., time to travel is longer.  Hence, these dispatchers will be removed from the active list after a fewer point assignments.

The quota of all dispatchers may be exhausted while some points remain unassigned.
QuotaBalanced re-computes the quota of each dispatcher using the remaining points, see Lines 16-18.  It continues to assigns points to the dispatchers until their quotas are exhausted.  This process repeats until all points are assigned to dispatchers.
The number of repetitions is 1393
with the point cloud of Section~\ref{sec:staticeval}.  

A dispatcher with no FLSs is permanently removed from the Active list (Lines 9-11).
This causes other dispatchers to deploy FLSs to render the illumination. 

The worst case complexity of this heuristic is O($\psi \times \alpha$).  It may perform fewer comparisons than MinDist because dispatchers are removed from the list.  At the same time, in each iteration, it performs more work when compared with MinDist because it must consider the travel time of an FLS to adjust the quota of a dispatcher and potentially reset the quota of all dispatchers.
In our experiments of Section~\ref{sec:staticeval}, MinDist and QuotaBalanced provided comparable execution times. 

Once points are assigned to dispatchers, a dispatcher may deploy FLSs similar to the discussion of MinDist, see Lines 19-21.  
%Similar to MinDist, its second for loop deploys FLSs.  This step may be performed by dispatchers in parallel similar to MinDist. 
There is one difference.  With QuotaBalanced, dispatchers may deploy FLSs that cross paths and potentially crash with one another.  Dispatchers may share the flight path and deployment time of their FLSs with one another to detect such potential crashes.  Prior to deploying an FLS, a dispatcher may detect a conflict with other deployed FLSs traveling to their target point.  It may implement a variety of techniques to prevent crashes.  
A simple technique is to delay the deployment of the FLS by the flight time of the conflicting FLS, increasing the latency to render an illumination. 
Alternatively, the dispatcher may compute a different flight path for its FLS, eliminating a possible crash.  


%%%A simple preventive technique will require the detecting dispatcher to delay deployment of its FLS by the flight time of the conflicting FLS, increasing the latency to render an illumination.  A more sophisticated technique may require the detecting dispatcher to compute a different flight path for its FLS, eliminating a possible crashes.  

\subsubsection{A Comparison}\label{sec:staticeval}

We use the Princeton Shape Benchmark~\cite{princetonbenchmark} to highlight the quantitative and qualitative differences between MinDist and QuotaBalanced.  Its database consists of 1,814 3D models.  We present results from 1 model, the race car (m1510), as the findings are identical across all models.  Figure~\ref{fig:m1510} shows the thumbnail for this model and its derived point cloud consisting of 11,894 points. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/m1510v2.png}
%\caption{Thumbnail of the point cloud m1510.}
\caption{Shape m1510, thumbnail and its point cloud.}
    \label{fig:m1510}
\end{figure}

We simulate an FLS display that is a cube with length=100, height=100, and depth=100 cells.  This display consists of 8 dispatchers, one at each corner of the cuboid.  Each dispatcher may deploy 10 FLSs per second, one FLS every 100 milliseconds.  The speed of each FLS is 4 cells per second.  An FLS flies along a straight line from the location of its dispatcher to the coordinates of its assigned point.

While QuotaBalanced uses all 8 dispatchers\footnote{The difference between the dispatcher that deploys the most number of FLSs and the one that deploys the fewest number of FLSs is 197, approximately 20\%.} to deploy FLSs, MinDist uses only 2 at the bottom corner\footnote{One deploys 6613 and the other deploys 5281 FLSs.} of the display.  Hence, QuotaBalanced enhances latency four folds, see 1st row of Table~\ref{tbl:staticCMP}.
This comes at a cost, namely, an increase in the total distance travelled by the FLSs.
This metric is more than 2x higher with
QuotaBalanced, see 2nd row of Table~\ref{tbl:staticCMP}.
This translates into a higher energy consumption to enhance latency.

QuotaBalanced exhausts the list of active dispatchers and resets their quota (Lines 16-18 of Alg~\ref{alg:balance}) 1393 times with this model.

Our simulated dispatchers detect when the path of their deployed FLSs intersect one another, identifying a conflict that may result in FLSs crashes.  
QuotaBalanced incurs 35 such conflicts.
Not every detected conflict is a crash because one FLS may fly past the crash point in advance of the other conflicting FLSs.  In our study, FLSs must be in 20\% proximity of one another to be considered as conflicting.
Table~\ref{tbl:staticCMP} shows QuotaBalanced incurs 12 such conflicts.  This is because dispatchers deploy FLSs that are farther away from a point in the display coordinate system than the other dispatchers.  This is a small percentage (0.1\%) of the 11,894 deployed FLSs by the 8 dispatchers.  See the last paragraph of the previous section on how to eliminate possible crashes.

%When a dispatcher deploys an FLS $i$, our simulator detects which of the previously deployed FLSs fall on its trajectory.  Each detected FLS $j$ is counted as a conflict with the potential to cause FLS crash.  The simulator resolves these conflicts by requiring (a) FLS $j$ to assume the identity of FLS $i$ and fly to the coordinates of the point illuminated by FLS $i$, and (b) FLS $i$ to assume the lighting responsibility of FLS $j$ and stop at the coordinates of FLS $j$.  The number of such conflicts are shown in the last row of Table~\ref{tbl:staticCMP}.  MinDist has zero conflicts because only two dispatchers deploy FLSs, each starting with its farthest away point (that is non-overlapping with the points of the other dispatcher).  QuotaBalanced observes a higher number of conflicts because its dispatchers deploy FLSs that cross each other's paths.    

\begin{table}
\begin{small}
  \caption{MinDist vs. QuotaBalanced}
  \label{tbl:staticCMP}
  \begin{tabular}{c|cc}
    \toprule
    & MinDist & QuotaBalanced\\
    \midrule
    Illumination Latency (Seconds) & 661 & 163 \\
    Distance Travelled (Cells) & 494,938 & 1,122,947\\
    Intersecting flight paths & 0 & 35 \\
    FLS Conflicts & 0 & 12 \\
    Execution Time (Milliseconds) & 27.71 & 27.44 \\
    %$\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
  \bottomrule
\end{tabular}
\end{small}
\end{table}


\subsection{Display of Motion Illuminations}
We assume a motion illumination consists of a sequence of point clouds displayed at a pre-specified rate.  
See 
%the Rose illumination of 
Figure~\ref{fig:intro:rosegrid}a.

%We focus on intra-scene point clouds with minimal changes from one point cloud to the next.
%For example, the Rose illumination of Figure~\ref{fig:intro:rose} with a falling petal consists of 115 point clouds.  Its display time is 4.79 seconds with 24 point clouds displayed per second. Each point cloud consists of approximately 65K points.

Assuming an FLS corresponds to a point, a display must compute both travel path of FLSs and their change of color from one point cloud $\Xi_i$ to the next point cloud $\Xi_{i+1}$.  While these changes may be minor with point clouds that constitute a scene, they may be drastic from the last point cloud of one scene to the first point cloud of its following scene.  This paper focuses on computing the intra-scene travel paths, deferring inter-scene travel paths to future work. 

To render a scene, the display must assign an FLS to each point of its first point cloud $\Xi_1$.  This is identical to rendering a static illumination.
Thus, either MinDist or QuotaBalanced maybe used.
To render its subsequent point cloud $\Xi_2$, the Orchestrator must compute whether:
\begin{enumerate}
    \item\label{simple:scenario1} $\Xi_2$ consists of more points than $\Xi_1$, requiring additional FLSs to render it.
    In general, dark FLSs from a previous point cloud (say $\Xi_{i-1}$) may be used to render $\Xi_{i+1}$.
    If none are available then FLSs are deployed by a dispatcher.
    \item\label{simple:fewer} $\Xi_2$ consists of fewer points than $\Xi_1$, requiring some FLSs illuminating $\Xi_1$ to either go dark or fly to a charging station.  Dark FLSs may be used in a subsequent point cloud, say $\Xi_3$.  This may minimize the overall distance travelled by FLSs.  This is because requiring FLSs to fly back to a charging station for $\Xi_2$ only to dispatch FLSs to illuminate $\Xi_3$ may result in a longer total travel distance. 
    \item\label{simple:colorchangeonly} An FLS illuminating $\Xi_1$ remains stationary and changes color in $\Xi_2$.
    \item\label{simple:flyoldnewcolor} An FLS illuminating $\Xi_1$ flies to a new point identified by $\Xi_2$ and displays either the same or a different color.
    %\item\label{simple:flynewcolor} A $\Xi_1$ FLS flies to a new position and displays a different color in $\Xi_2$.
    \item\label{simple:nochange} An FLS illuminating $\Xi_1$ remains stationary and continues to display its current color in $\Xi_2$.  This is the scenario where the point in $\Xi_1$ and $\Xi_2$ are identical, i.e., identify the same illumination cell and render the same color.
\end{enumerate}
Any and all combinations of these possibilities may apply when considering two point clouds $\Xi_i$ and $\Xi_{i+1}$.
%%%A point cloud of the Rose illumination consists of 65K points.  All the above possibilities may be present when considering two point clouds $\Xi_i$ and $\Xi_{i+1}$ of this clip.

This section presents two offline algorithms, Simple and Motill, to detect the alternative scenarios and compute FLS flight paths and color renderings.
Similar to the MPEG encoding technique, a system may execute these algorithms once for a motion illumination, store their computed flight paths, and reuse this information when rendering a motion illumination repeatedly either for the same user or different users.  

\subsubsection{Simple}\label{sec:simple}
Simple is an offline algorithm that consists of two steps.
%Step 1 computes the flight path of FLSs between all pairs of point clouds $\Xi_i$ and $\Xi_{i+1}$ that constitute a scene.  This step computes a set of flight paths $\{\epsilon_i\}$ for point cloud $\Xi_i$.  These flight paths navigate a subset (potentially all) FLSs that are rendering $\Xi_i$ to illuminate $\Xi_{i+1}$.  %Step 1 identifies those FLSs of $\Xi_i$ that are extras.  We use set $\{\delta_i\}$ to denote these FLSs.  
%Step 1 also identifies those FLSs of $\Xi_i$ that are extras, $\{\delta_i\}$, and those points of $\Xi_{i+1}$ that have no assigned FLSs, $\{\mu_{i+1}\}$. 
Step 1 computes flight paths that transition one point cloud to the next.  It also identifies FLSs that are extras from one point cloud to next.  And, points that may require FLSs to be deployed by a dispatchers.
More formally, with $n$ point clouds, $\{\Xi_1, \Xi_2, \cdots, \Xi_n\}$, Step 1 computes four sets.
Flight paths for the first $n-1$ point clouds, denoted $\{\epsilon_1, \epsilon_2, \cdots, \epsilon_{n-1}\}$.
Change of color for the FLSs used in the first $n-1$ point clouds, denoted $\{\gamma_1, \gamma_2, \cdots, \gamma_{n-1}\}$.
Extra FLSs for the first $n-1$ point clouds, denoted $\{\delta_1, \delta_2, \cdots, \delta_{n-1}\}$.
There are extra FLSs when $\Xi_i$ consists of more FLSs than $\Xi_{i+1}$.
Points with no assigned FLSs for the last $n-1$ point clouds, denoted $\{\mu_2, \mu_3, \cdots, \mu_{n}\}$.
$\Xi_i$ may have points with no assigned FLSs when it consists of more points than $\Xi_{i-1}$.

In Step 2, Simple processes $\{\delta_i\}$ to decide whether one or more of its FLSs should stay in the display grid and go dark or fly back to a charging station.  The dark FLSs are assigned to a point identified by a $\{\mu_{j>i}\}$.  Step 2 may schedule a dispatcher to deploy FLSs to illuminate points of $\{\mu_j\}$.

Step 2 is required when there are extra FLSs, points with no assigned FLSs, or both, i.e., either $\{\delta_i\}$, $\{\mu_j\}$, or both are not empty.
Step 1 produces empty $\{\delta_i\}$ and $\{\mu_j\}$ when the different point clouds consist of the same number of points.  In this case, Simple does not execute Step 2.

Simple may optimize for total distance travelled, the amount of energy used, the time required to execute flight paths, or a hybrid of these.  The hybrid may assign weights to different criterion.  This paper focuses on minimizing the total distance travelled by FLSs, deferring other possibilities to future work.  Below, we detail the two steps in turn.

%%Simple processes two point clouds $\Xi_i$ and $\Xi_{i+1}$ to detect and resolve the different scenarios.
%%%It resolves Scenarios~\ref{simple:scenario1}-\ref{simple:flyoldnewcolor} by computing flight paths for some FLSs belonging to $\Xi_i$ to illuminate $\Xi_{i+1}$. 
%%Its objective is to minimize the total distance travelled by the FLSs.
%%This includes distance travelled by FLSs that return to a charging station or deployed by a dispatcher.
%flights by FLSs deployed by a dispatcher or returned to a charging station.

%%\subsubsection{Detection of different scenarios} 
In Step 1, Simple constructs a hash table on the coordinates of $\Xi_i$ and probes it with coordinates of $\Xi_{i+1}$.  For each match, it checks whether the color of the probing point is the same or different.  If they are the same, it has identified a point that belongs to Scenario~\ref{simple:nochange}.
If different then it has identified a point that belongs to Scenario~\ref{simple:colorchangeonly}.
It adds this change to $\gamma_i$.

If the point from $\Xi_{i+1}$ has no match then it is added to the set $\{\mu_{i+1}\}$.  This point is a candidate for Scenario~\ref{simple:flyoldnewcolor} if $\Xi_{i}$ and $\Xi_{i+1}$ consist of the same number of points.
It is a candidate for Scenario~\ref{simple:scenario1} (Scenario~\ref{simple:fewer})
if $\Xi_{i}$ has more (fewer) points than $\Xi_{i+1}$.

Step 1 constructs $\{\delta_i\}$ as follows.  It deletes a hash table entry that matches a coordinate of $\Xi_{i+1}$.
Once all points of $\Xi_{i+1}$ have probed the hash table, 
Simple enumerates those points that remain in the hash table and assigns them to $\{\delta_i\}$.
FLSs in $\{\delta_i\}$ correspond to $\Xi_i$ points with no matches in $\Xi_{i+1}$.
%They are used to render $\Xi_i$ and are freed in $\Xi_{i+1}$.
%Simple may require these to fly to a new coordinate and change color (includes going dark) to render a point of $\Xi_{i+1}$ that appears in $\{\mu_{i+1}\}$, addressing Scenarios~\ref{simple:fewer} and~\ref{simple:flyoldnewcolor}.
%With those that address Scenario~\ref{simple:flyoldnewcolor}, some may go dark to address the same scenario for a subsequent point cloud, say $\Xi_{i+2}$.  This is handled in this step as detailed below.

%that identifies those FLSs that change their position from point cloud $C_i$ to the next point cloud $C_{i+1}$ and computes their flight paths.  Its objective is to minimize the total distance travelled by FLSs.

%Given two point clouds that follow one another in a scene, $C_i$ and $C_{i+1}$, a simple technique may compute those points whose position does not change from $C_i$ to $C_{i+1}$.  Next, it identifies points present $C_i$ and missing from $C_{i+1}$, $\delta_i$.  And, identify points present in $C_{i+1}$ and missing from $C_i$, $\delta_{i+1}$.  If the number of points in $\delta_i$ is greater than $\delta_{i+1}$ then some FLSs must either go dark or fly back to a dispatcher.  If the number of points $\delta_i$ is less than $\delta_{i+1}$ then either dark in-flight FLSs of $C_i$ must start to render color or dispatchers must deploy FLSs to render missing points of $C_{i+1}$.  

Step 1 computes flight paths by mapping points of $\{\delta_i\}$ to $\{\mu_{i+1}\}$.
It minimizes the overall distance using the following greedy heuristic.
It computes the distance\footnote{Distance may be replaced with the amount of energy required or flight time to consider different objectives.} between every pairing of a $\{\delta_i\}$ point with a $\{\mu_{i+1}\}$ point.  
It sorts these pairing in ascending distance.
It selects the first pairing, ($P_{1,\delta},P_{1,\mu}$), and assigns the FLS at the display cell $P_{1,\delta}$ to fly to the vacant display cell identifies by $P_{1,\mu}$ that requires illumination.
This is a flight path with a source coordinate $P_{1,\delta}$ and a destination coordinate $P_{1,\mu}$ that transitions $\Xi_i$ to render $\Xi_{i+1}$.
It is added to the set of flight paths $\{\epsilon_i\}$.
%It adds this flight path to its list of FLS fly paths for $\Xi_{i}$.  
Simple removes the coordinates $P_{1,\delta}$ and $P_{1,\mu}$ from its sorted list of possibilities, and 
from $\{\delta_i\}$ and $\{\mu_{i+1}\}$, respectively.
Step 1 continues with the next pairing, repeating this process until either $\{\delta_i\}$, $\{\mu_{i+1}\}$, or both are empty.

If both $\{\delta_i\}$ and $\{\mu_{j}\}$ are empty then Simple terminates.  Otherwise, it proceeds to Step 2.

Step 2 processes $\{\delta_i\}$ and $\{\mu_{j}\}$ sets.
If $\{\delta_i\}$ is not empty and $\{\mu_{j}\}$ is empty then all FLSs in $\{\delta_i\}$ are required to fly back to a charging station after rendering their point cloud $\Xi_i$.
If $\{\mu_j\}$ is not empty and $\{\delta_i\}$ is empty then dispatchers are scheduled to deploy FLSs to points identified by $\{\mu_j\}$ to illuminate point cloud $\Xi_j$.
With both scenarios, Step 2 is complete and Simple terminates.
%Below, we detail Step 2 when both $\{\delta_i\}$ and $\{\mu_j\}$ are not empty.

When both $\{\delta_i\}$ and $\{\mu_{j}\}$ are not empty then Step 2 processes the two sets as follows.
If there is a $\{\delta_i\}$ with no following $\{\mu_{j}\}$ ($i < j$) then all FLSs identified by $\{\delta_i\}$ are scheduled to fly back to a charging station.  Otherwise, Step 2 computes the distance\footnote{Distance may be replaced with the amount of energy required or flight time to consider different objectives.} between every pairing of a $\{\delta_i\}$ point with a $\{\mu_{j}\}$ point.
It sorts these pairing in ascending distance.
It selects the first pairing, ($P_{1,\delta},P_{1,\mu}$) with distance $\tau_1$, and computes the total distance travelled if $P_{1,\delta}$ flies to a charging station and an FLS is deployed by a dispatcher closest to $P_{1,\mu}$ to illuminate $P_{1,\mu}$.  If the total distance is smaller than $\tau_1$ then the FLS identified by $P_{1,\delta}$ is scheduled to fly back to a charging station\footnote{In this scenario, Step 2 may consider other following $\mu_{k>j}$.  This may identify a destination point in a point cloud $\Xi_k$ for the FLS in $\delta_i$, producing a flight path stored in $\epsilon_i$.}.
Otherwise, Step 2 computes the flight path from $P_{1,\delta}$ to $P_{1,\mu}$ and adds this path to $\epsilon_i$.
Step 2 removes $P_{1,\delta}$ and $P_{1,\mu}$ from its sorted table, and from $\delta_i$ and $\{\mu_{j}\}$, respectively.

Step 2 processes other special cases not detailed here.  For example, if there is a $\{\mu_{j}\}$ with no preceding $\{\delta_i\}$ ($i<j$) then Step 2 schedules FLSs to be deployed by a dispatcher to illuminate points identified by $\{\mu_{j}\}$.

%If $\{\delta_i\}$ is not empty then its FLSs are added to $\{\delta_{i+1}\}$.  
%These FLSs are candidates to go dark and may be used to render a future point cloud $\Xi_j$, $j>i+1$.
%Whether they are chosen in this role or required to fly back to a charging station is decided in Step 2.

%Once Step 1 completes, Simple has three variables associated with point cloud $\Xi_i$:  a set of flight paths $\{\epsilon_i\}$, $\{\delta_i\}$ idle FLSs in point cloud $\Xi_i$, and $\{\mu_{i}\}$ missing FLSs from $\Xi_{i-1}$.  The last point cloud of the scene is the exception.

%In Step 2, Simple analyzes $\{\delta_i\}$ associated with each point cloud $\Xi_i$ as follows.  If $\{\delta_i\}$ is empty then it is deleted.  If it identifies one or more FLSs then, for each FLS, Simple looks ahead to see if the FLS is used in a future point cloud $\Xi_j$, $j>i+1$.  If the FLS is not used then it must fly back to a charging station.  If the FLS is used then Simple determines whether the distance is minimized by maintaining the FLS in flight (Scenario~\ref{simple:fewer}) or having it fly back to a charging station. With the latter, an FLS must be deployed by a dispatcher and its traveled distance is considered in our analysis.

%Step 2 may use the amount of energy consumed by FLSs (instead of distance) to decide whether a $\delta_i$ FLS should remain in the display or fly back to the charging station.

%Step 2 terminates once there is no point cloud $\Xi_i$ with a $\{\delta_i\}$ set.
%Once there are no more $\{\delta_i\}$ sets remain, Step 2 terminates.  The final flight paths for each point cloud is stored in a file to render an illumination. When rendering the illumination using this file, a display applies flight paths of $\epsilon$ to FLSs of $\Xi_i$ to render $\Xi_{i+1}$.  These flight paths are provided to each individual FLS for as many point clouds accommodated by its storage.  Periodically, the FLS polls the Orchestrator for its remaining flight paths.

%FLSs identified in $\delta_i$ may appear in a $\delta_j$ ($j>i$), identifying their use to render a future point cloud.  Those that do not must fly back to a charging station.

%$\delta_i$ FLSs that appear in a $\delta_j$ are further processed to determine whether distance is minimized by maintaining them in flight (Scenario~\ref{simple:fewer}) or flying them back to a charging station.  With the latter, an FLS must be deployed by a dispatcher and its traveled distance is considered in our analysis.

%This generates a 3 column table with a source coordinate from $\delta_i$, a destination coordinate in $\delta_{i+1}$, and flight distance.  Next, it sorts these pairings in ascending flight distance order.  It assigns the first pairing, (Source, Destination, Distance), to the FLS at the Source coordinate of $\Xi_i$.  Next, it computes the flight path for the FLS at the Source to the Destination at $\Xi_{i+1}$.  It deletes all those rows of the sorted table with Source as their first column value.  It also deletes those rows with Destination as their second column value.  The algorithm repeats this process to compute flight paths for other FLSs in $\Xi_i$.  It terminates once the sorted table is empty.


\subsubsection{An Analysis}\label{sec:simpleanalysis}
In our experiments with the Rose illumination, Step 1 requires approximately 600 seconds to compute flight paths for FLSs that constitute two consecutive point clouds.  
This step wastes time and resources by computing a pairing of each FLS in $\{\mu_{i+1}\}$ with each FLS in $\{\delta_i\}$ to identify the pairing with the shortest distance.  Only one qualifies.  Step 1 must find and delete the remaining $|\{\mu_{i+1}\}|-1$ possibilities.

Step 1 is not optimal even though it enumerates all possible mappings from FLSs in $\{\delta_i\}$ to the vacant coordinates in $\{\mu_{i+1}\}$.  This is trivial to demonstrate with an example.
Assume $\{\delta_i\}$=$\{P_1,P_2\}$ and $\{\mu_{i+1}\}$=$\{Q_1,Q_2\}$.
Assume distance from $P_1$ to each of $Q_1$ and $Q_2$ is 1 and 2 cells, respectively.  And, distance from $P_2$ to each of $Q_1$ and $Q_2$ is 2 and 5 cells, respectively.
The optimal minimum distance of 4 is realized by flying the FLS located at $P_1$ to the coordinates of $Q_2$, and flying the FLS at $P_2$ to the coordinates of $Q_1$.
However, Step 1 maps $P_1$ to $Q_1$ because their distance is the smallest.
It must subsequently map $P_2$ to $Q_2$, resulting in 6 as the total travelled distance by FLSs at $P_1$ and $P_2$.
This example demonstrates Step 1 of Simple does not compute optimal pairings of FLSs in $\{\delta_i\}$ and $\{\mu_{i+1}\}$.

\subsubsection{Motion Illuminations, Motill, Encoding}\label{sec:motill}
Motill is a family of divide-and-conquer encoding techniques to implement Step 1 of Simple.
%They detect and resolve Scenarios~\ref{simple:scenario1}-\ref{simple:flyoldnewcolor} between two point clouds $\Xi_i$ and $\Xi_{i+1}$.
%They assume an FLS rendering a point in $\Xi_i$ travels a short distance to render a different point in $\Xi_{i+1}$.
They localize mapping of the points by constructing a 3D grid on the point clouds.
Instead of computing the distance between a freed FLS of $\Xi_i$, $\{\delta_i\}$, with every vacant coordinate of $\Xi_{i+1}$, $\{\mu_{i+1}\}$, Motill compares those in the same cuboid or its neighboring cuboids.  Other pairings are guaranteed to be farther away.  By eliminating them from consideration, Motill reduces complexity of Step 1 to provide a faster execution time when computing FLS flight paths.
In addition, 
a Motill technique named ICF provides shorter flight distances for FLSs when compared with Simple. 

Motill is highly parallelizable and may use multiple cores of a processor to compute flight paths, see Section~\ref{sec:parallel}.
Simple is a special case of Motill with a grid consisting of 1 cuboid, see Section~\ref{sec:motillandsimple}.

Both lossy and lossless variants of Motill are possible.  In lossy mode, Motill may remove certain points to minimize the number of FLSs used to render an illumination.  In lossless mode, the number of FLSs is the same as the number of points.  The focus of this papers is on the lossless Motill. 

Motill partitions a scene consisting of $n$ points clouds into a Group of Point Clouds (GPCs).
Each GPC consisting of $\omega$ point clouds, $\{\Xi_1, \Xi_2, \cdots, \Xi_\omega\}$, $\omega \leq n$.  A point in a GPC corresponds to an FLS.  Motill computes flight paths for different FLSs across a GPC $\{\Xi_1, \Xi_2, \cdots, \Xi_\omega\}$.  Subsequently, Motill combines flight paths computed for the different GPCs together to compute the travel path of FLSs for the entire scene.

Motill processes a GPC by constructing a 3D grid on its first point cloud $\Xi_1$.  A maximum limit $\theta$ is imposed on the number of points assigned to each cuboid of the grid.  Every time a cuboid overflows, Motill breaks the cuboid into two by partitioning it along a dimension.  In our current implementation, we use a round-robin policy to select among the dimensions across all cuboids.  However, it is possible to develop more sophisticated policies to better balance points across the cuboids. 

Motill constructs a copy of the $\Xi_1$ grid with $\rho_1$ cuboids on the remaining point clouds of a GPC, $\Xi_2$ to $\Xi_\omega$.
%Motill superimposes a copy of the $\Xi_1$ grid with $\rho$ cuboids on the remaining point clouds of a GPC, $\Xi_2$ to $\Xi_\omega$. 
It scans points of $\Xi_i$ ($1 < i \leq \omega$) and assigns each to the cuboid that contains it, populating $\Xi_i$ grid.
%%It populates the grid copy of $\Xi_i$ ($i>1$) by scanning its points and assigning each point to the cuboid that contains it.
This step does not detect overflows and has no cuboid splits.
Hence, the cuboids of these point clouds may have more points than the maximum limit $\theta$.

The purpose of the grid is to reduce the number of points considered when computing the shortest distance.  Its cuboids localize how a point (FLS) changes position from one point cloud to the next.  By using the same grid across all point clouds of a GPC, Motill localizes changes to a few cuboids.
To describe how this is accomplished, 
%%%see Section~\ref{sec:gridprocessing}. 
we define the terms grid and neighboring cuboids.  We use these terms in the following section that details Motill's processing of the grid.
%%%describe how Motill uses the grid to detect Scenarios~\ref{simple:scenario1}-\ref{simple:flyoldnewcolor} and compute FLS flight paths to address them.

%\begin{definition}
%A cuboid consists of six flat faces and eight vertices.  All its faces are rectangles.  A cuboid is a square prism when at least two faces are squares.  A cuboid is a cube when all its six faces are squares.  
%A Motill grid may consist of a mix of cuboids, square prisms, and cubes.  We use the term cuboid to refer to an element of a grid even though it may be a cube or a square prism.  
%\end{definition}

\begin{definition}
A grid is a 3-dimensional coordinate space consisting of a fixed number of cuboids $\rho$.  
\end{definition}

\begin{definition}\label{def:neighbor}
Two cuboids of a grid are neighbors if their coordinate spans 
overlap along 2 dimensions (i.e., share a 2D face either partially or fully) and abut along one dimension.   
\end{definition}
%For example, in Figure~\ref{fig:intro:rosegrid}b, Cuboid 2 is neighbors with 1, 3, and 5.  Cuboid 3 has all the shown cuboids as its neighbor.  

\subsubsection{Grid processing}\label{sec:gridprocessing}
Motill processes the cuboids that constitute the grid of $\Xi_1$ to $\Xi_\omega$ to compute FLS flight paths, $\{\epsilon_1, \epsilon_2, \cdots, \epsilon_{\omega-1}\}$.  It processes two sequential point clouds, $\Xi_i$ and $\Xi_{i+1}$, by enumerating their respective cuboids and processing one pair at a time.
We identify one such pairing as $C_i^j$ and $C_{i+1}^j$.  The subscript identifies the point cloud and the superscript identifies the cuboid.  A pairing must have the same superscript value, i.e., identify the same cuboid in two consecutive point clouds with identical L, H, and D dimensions and neighbors.




% \begin{enumerate}
    % \item No change: $C_i^j$ and $C_{i+1}^j$ have the same number of points.  Both the L, H, D coordinate of each point and its color is the same across both cuboids.
    
    % \item Color change: $C_i^j$ and $C_{i+1}^j$ have the same number of points and the coordinates of their points is identical.  However, the color of some points is different.
    
    % \item Position change: While $C_i^j$ and $C_{i+1}^j$ have the same number of points and the color of these points is identical, the L, H, D coordinates of some points is different.
    
    % \item Different number of points:  The coordinates of the points and their color is the same for $C_i^j$ and $C_{i+1}^j$.  However, the number of points is different.  $C_i^j$ has either more or fewer points than $C_{i+1}^j$. 
    
    % \item Any combination of the previous three possibilities.  Six combinations are possible.  One has all three changes where $C_i^j$ and $C_{i+1}^j$ having different number of points, and position and color of some points change from $C_i^j$ to $C_{i+1}^j$.  
% \end{enumerate}

Motill uses Simple's Step 1 hashing technique to detect Scenarios~\ref{simple:scenario1}-\ref{simple:flyoldnewcolor}
for each cuboid pair $C_i^j$ and $C_{i+1}^j$.
With Scenario~\ref{simple:flyoldnewcolor},
it constructs $\{\delta_i^j\}$ and $\{\mu_{i+1}^j\}$ for each pairing
per discussions of Step 1, see Section~\ref{sec:simple}.

Motill computes intra-cuboid and inter-cuboid flight paths to transition FLSs of $\Xi_i$ to illuminate $\Xi_{i+1}$.
Intra-cuboid flight paths are local to cuboids $C_i^j$ and $C_{i+1}^j$.
Inter-cuboid flight paths may be in two from:  FLSs from a different cuboid in $\Xi_{i}$ flying into $C_{i+1}^j$ or FLSs from $C_i^j$ flying to a different cuboid in the point cloud $\Xi_{i+1}$.

%It computes intra-cuboid flight paths from a $C_i^j$ point to a $C_{i+1}^j$ point.  It computes inter-cuboid flight paths for FLSs that fly either from a different cuboid to $\Xi_{i+1}$'s $C_{i+1}^j$ or from $\Xi_i$'s $C_i^j$ to a different cuboid of $\Xi_{i+1}$.

Motill computes intra-cuboid flight paths by processing $\{\delta_i^j\}$ and $\{\mu_{i+1}^j\}$ using Simple, i.e., enumerating all possible combinations, sorting, and selecting the one with the shortest distance for its flight path.  
It computes inter-cuboid flight paths by identifying those cuboids of $\Xi_{i+1}$ that have more points than their respective $\Xi_i$ cuboids and those cuboids of $\Xi_{i+1}$ with fewer points than their respective $\Xi_i$ cuboids.  This results in two sets of cuboids, $\{C^+\}$ and $\{C^-\}$.  It processes one cuboid of $\{C^+\}$ by identifying its neighbors %(see Definition~\ref{def:neighbor}) 
to determine which appears in the set $\{C^-\}$.  For each such cuboid, it computes all possible mappings to select a destination point with the shortest distance.  

It is possible that there is no neighboring cuboid that intersects a cuboid in set $\{C^-\}$.  Motill collects these and in a final pass enumerates the points in cuboids of $\{C^+\}$ and points in cuboids of $\{C^-\}$.  It uses Simple's technique to map these points together, computing flight paths for FLSs.  

\subsubsection{Variants of Motill}\label{sec:variants}
Motill is a family of techniques.  In this paper, we consider two variants:  Intra-Cuboid-First (ICF) and Intra-Cuboid-Last (ICL).
ICF computes intra-cuboid flight paths for every cuboid pairing first.
For the remaining cuboids, it computes inter-cuboid flight paths.  It is motivated by the insight that computing flight paths local to a cuboid minimizes distance.

ICL reverses the order of these two steps, computing inter-cuboid flight paths first and intra-cuboid flight paths last.
Its motivation is that computing inter-cuboid flight paths first has the benefit of more candidate FLSs in $\{\delta_i^j\}$ and vacant destinations in $\{\mu_{i+1}^j\}$.
%ICF imposes a higher constraint on the inter-cuboid flights by removing candidates from $\delta_i^j$ and $\mu_{i+1}^j$.  

%With both variants, Motill has a final step for two consecutive points clouds, $\Xi_i$ and $\Xi_{i+1}$, with varying number of points.  Its computation identifies either cuboids of $\Xi_i$ with FLSs that are no longer needed in $\Xi_{i+1}$ or cuboids of $\Xi_{i+1}$ that require FLSs.  With the former, Motill may maintain the extra FLSs and require them to go dark, using them for the subsequent point cloud $\Xi_{i+2}$.  With the latter, Motill may either deploy FLSs from a dispatcher or use dark FLSs from $\Xi_{i+1}$.

Both ICF and ICL implement Step 2 of Simple.
%%% that considers the $\delta_i$ associated with every point cloud $\Xi_i$ to decide whether extra FLSs fly to a charging station or go dark for use by a future point cloud. 
Experimental results of Section~\ref{sec:evalmotill} show ICF is superior to ICL for the Rose illumination.
It executes faster and minimizes the total distance travelled by FLSs.  

\subsubsection{Parallelism}\label{sec:parallel}  
Motill variants may employ parallelism at different granularity, using multi-core CPUs with minimal coordination.
First, they may process different GPCs that constitute a scene in parallel.
A challenge is how to fuse travel paths computed for two consecutive GPCs, $\varphi_1$ and $\varphi_2$.
%There are several possible ways to fuse travel paths computed for two consecutive GPCs, $\varphi_1$ and $\varphi_2$.
%If each point of a point cloud is identified with a unique identifier across the point clouds then the task is trivial.  Motill simply takes the travel path computed for each unique point (FLS) of $\varphi_1$ and $\varphi_2$ in a sequence and merges them into one.  If no unique identifier exists then Motill may
A simple technique is to repeat the last point cloud $\Xi_\omega$ of $\varphi_1$ as the first point cloud $\Xi_1$ of $\varphi_2$.
%use the coordinates of the points in the last point cloud $\Xi_\omega$ of $\varphi_1$ to identify the corresponding points in the first point cloud $\Xi_1$ of $\varphi_2$.  
%The complexity of this matching task may be reduced by using the last point cloud $\Xi_\omega$ of $\varphi_1$ as the first point cloud $\Xi_1$ of $\varphi_2$.  
This reduces the matching task to a simple 3D coordinate lookup of the first point cloud $\Xi_1$ of $\varphi_2$ using the coordinates of the last point cloud $\Xi_\omega$ of $\varphi_1$.  For each match, the travel path for an FLS in $\varphi_1$ is concatenated with travel path from $\varphi_2$ after removing the redundant path attributed to the repeated use of $\Xi_\omega$ of $\varphi_1$.

Second, Motill may populate
the grids on $\Xi_2$ to $\Xi_\omega$ in parallel, using a different core for each point cloud.
(Recall from Section~\ref{sec:gridprocessing} that the structure of these grids is a copy of $\Xi_1$ grid.)  

Third, Motill may compute intra-cuboid flight paths for the different cuboids in parallel.  With hundreds of cuboids in a grid, Motill may use hundreds of cores concurrently.  Parallel processing of inter-cuboid flight paths requires an extra pre-processing step to identify those cuboids considered concurrently to not share neighbors.  %It is trivial for Motill to quantify the number of FLSs that may be removed or added to a cuboid by analyzing its number of points across the point clouds $\Xi_1$ and $\Xi_{i+1}$.

Motill may use the concept of stragglers to enhance latency.  Given a thousand core processor, assuming certain cores are idle, Motill may use these cores to execute a copy of tasks that are taking too long to complete (consuming the result of the copy that finishes first).
Stragglers waste computing resources by performing redundant work to enhance latency.

\subsubsection{Motill and Simple}\label{sec:motillandsimple}
%MOVE TO THE END OF THIS SECTION?
Motill with one cuboid emulates Simple.
We realize this by setting the capacity of a cuboid to a large number, i.e., maximum integer value.  This transforms the different variants of Motill to employ simple for intra-cuboid mappings.

Motill is faster than Simple.  
When configured with a reasonable number of cuboids for its grid, Motill also provides better flight paths that minimize total travelled distance.
We quantify this in the next section. %Section~\ref{sec:evalmotill}.

\subsubsection{A Comparison}\label{sec:evalmotill}
This section compares Simple, ICF, and ICL using the Rose illumination of Figure~\ref{fig:intro:rosegrid}a.
This comparison uses the same software, an implementation of Motill, for all three techniques.
An input parameter of Motill switches the order of intra-cuboid processing to be either first or last.  We emulate Simple by setting the capacity of Motill cuboids to the maximum integer value to force it to construct one cuboid.
We quantify both the execution time of an algorithm and the total distance of its computed flight paths.  The actual execution of the flight paths by FLSs to render an illumination and its latency is a part of our future work.

The reported execution times for Simple do not include the time to construct Motill's one cuboid grid.
With ICF and ICL, the reported execution times include the grid construction times.

All reported execution times were gathered from MATLAB R2022a (9.12.0.1884502) running on a MacBook Pro configured with a 2.3 GHz 8-Core Intel i9 processor and 16 GB of memory.
Its operating system is macOS Big Sur Version 11.5.2.
All the data was staged in memory prior to gathering execution times, eliminating disk I/O times.
While obtained results are written to disk, this is performed at the end after the experiment timing has stopped.
Reported experiments did not use parallelism.


Main lessons are as follows:
\begin{itemize}
    \item ICF's computed flight paths provide a shorter total flight distance when compared with ICL.  Its execution time is faster for almost all point cloud pairings.  In those few cases that it is slower, the percentage difference is less than 4\%.  See discussions of Figure~\ref{fig:eval:ICLvsICFtime}.
    
    \item Simple is slower than both ICF and ICL.  With some point clouds, ICF is 5.5 to 6x faster than Simple.  See discussions of Figures~\ref{fig:eval:ICLvsICFtime} and~\ref{fig:eval:cubeSZtime}. 
    
    \item ICF provides comparable flight distances to Simple for most but not all pairs of point clouds.  See discussions of Figures~\ref{fig:eval:ICLvsICFdist} and~\ref{fig:eval:cubeSZdist}.
    
    \item Motill's cuboid size impacts its execution time and computed flight distances.  This is true with both ICF and ICL.  See discussions of Figure~\ref{fig:eval:cubesize}.
    
    \item With the Rose illumination, once FLSs are deployed using either MinDist or QuotaBalanced, the flight paths computed by the different techniques do not result in collisions.  Hence, no FLS collisions are reported.
    
    \item The point clouds that constitute the Rose illumination have the same number of points (65,321).  Hence, Simple and Motill do not execute their Step 2.
\end{itemize}

\begin{figure}
\begin{subfigure}[t]{0.47\columnwidth}
\centering
\includegraphics[width=\textwidth]{figs/ICLvsICFdistance.png}
\caption{Flight Distance.}
\label{fig:eval:ICLvsICFdist}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.47\columnwidth}
\centering
\includegraphics[width=\textwidth]{figs/ICLvsICFexecTime.png}
\caption{Execution Time.}
\label{fig:eval:ICLvsICFtime}
\end{subfigure}
\caption{%%%Throughput as a function of $\beta$ with 
ICL vs. ICF, cuboid size ($\theta$) is 1500 points/FLSs.}
\label{fig:eval:ICLvsICF}
\end{figure}

%\subsubsubsection{ICL vs. ICF}\label{sec:icl}
\noindent{\bf ICF vs. ICL:}
Figure~\ref{fig:eval:ICLvsICFdist} shows the flight distance computed by ICL and ICF.
The x-axis identifies the point cloud in the Rose illumination.  We used the 20$^{th}$ point cloud to the 33$^{rd}$ point cloud.
The y-axis shows the total distance of the flight paths computed by different techniques to transition from rendering point cloud $i$ (say 20) to the next point cloud $i+1$ (21).  All techniques compute the same number of flight paths (2009) for each point cloud. 


Figure~\ref{fig:eval:ICLvsICF} highlights several observations.
First, ICF results in a lower flight distance for all point clouds.
Second, ICF is faster than ICL for most but not all the point clouds, see Figure~\ref{fig:eval:ICLvsICFtime}.
It is slightly (<4\%) slower than ICL for the 33rd point cloud.
Third, the point cloud data impacts FLS flight distances and Motill execution times significantly.
It is interesting to note that the flight distance of ICF increases linearly with the first 14 point clouds, see Figure~\ref{fig:eval:cubeSZdist}.
And, the total distance for each of these points is lower than that of point clouds 20-26 of Figure~\ref{fig:eval:ICLvsICF}.
The y-axis scale is different for Figures~\ref{fig:eval:ICLvsICFdist} and~\ref{fig:eval:cubeSZdist}.

%%%Both metrics vary for different point clouds.  To illustrate, compare the metrics reported for ICF in Figure~\ref{fig:eval:ICLvsICF} with those reported in Figure~\ref{fig:eval:cubesize}.  (Compare the blue lines in the presented graphs.)  They are different because Figure~\ref{fig:eval:cubesize} reports results for the point clouds 1 to 14. 


\begin{figure}
\begin{subfigure}[t]{0.47\columnwidth}
\centering
\includegraphics[width=\textwidth]{figs/ICFsizeDist.png}
\caption{ICF Flight Distance.}
\label{fig:eval:cubeSZdist}
\end{subfigure}
\quad
\begin{subfigure}[t]{0.47\columnwidth}
\centering
\includegraphics[width=\textwidth]{figs/ICFsizeTime.png}
\caption{ICF Execution Time.}
\label{fig:eval:cubeSZtime}
\end{subfigure}
\caption{%%%Throughput as a function of $\beta$ with 
ICF with different cuboid size ($\theta$) values.}
\label{fig:eval:cubesize}
\end{figure}

\noindent{\bf Cuboid size:}
The cuboid size impacts Motill's execution time and computed flight distances, see Figure~\ref{fig:eval:cubesize}.
It dictates the structure of the grid and the number of cuboids that constitute it.
A small cuboid size results in a large number of cuboids and slow execution times.
A large cuboid size is also undesirable because it results in a few cuboids and starts to approximate Simple.
It computes many combinations of possible flight paths only to select one.
 
Figure~\ref{fig:eval:cubesize} highlights this using ICF with the 1$^{st}$ to 14$^{th}$ point clouds of the Rose illumination.
We report on cuboid sizes 100, 1500, 10K, and max integer (1 cuboid).
(The latter is Simple.)
Cuboid size 1500 provides the fastest execution times, see Figure~\ref{fig:eval:cubeSZtime}.  Moreover, its computed flight distances are comparable if not better than Simple, see Figure~\ref{fig:eval:cubeSZdist}.

In Figure~\ref{fig:eval:cubesize}, 
$\theta=100$ results in 987 cuboids.
The portion of execution time used by ICF is 18\%.  The rest of the time is spent constructing and copying the grid.  It is interesting to note that the time to copy and populate the grid with point clouds 2 to 14 is approximately the same as constructing the grid on point cloud 1.

In contrast, $\theta$=1500 constructs 68 cuboids.  Its time to construct the grid on the first point cloud is twice the time to copy it on the remaining point clouds.  Both are approximately 6x faster than $\theta$=100. The portion of execution time used by ICF increases to approximately 75\%. 

A large cuboid size, $\theta$=10,000, constructs only 10 cuboids.
It spends 90\% of its time computing possible flight paths that it subsequently discarded.

Note that $\theta$=10,000 computes competitive flight paths comparable to those of $\theta$=1,500 and is superior to Simple, see Figure~\ref{fig:eval:cubeSZdist}.
It also provides execution times that are at least 3x faster than simple, see Figure~\ref{fig:eval:cubeSZtime}.

Simple is the extreme cuboid size, resulting in a grid with one cuboid.
Its execution time is the highest in Figure~\ref{fig:eval:cubeSZtime}.
It does not incur the overhead of constructing a grid.
Instead, 
it wastes time and resources by computing many FLS flight paths that are subsequently deleted.  See discussions of Section~\ref{sec:simpleanalysis}.
